DensePeds: Pedestrian Tracking in Dense Crowds Using Front-RVO and Sparse Features

We present a pedestrian tracking algorithm, DensePeds, that tracks individuals in highly dense crowds (greater than 2 pedestrians per square meter). Our approach is designed for videos captured from front-facing or elevated cameras. We present a new motion model called Front-RVO (FRVO) for predicting pedestrian movements in dense situations using collision avoidance constraints and combine it with state-of-the-art Mask R-CNN to compute sparse feature vectors that reduce the loss of pedestrian tracks (false negatives). We evaluate DensePeds on the standard MOT benchmarks as well as a new dense crowd dataset. In practice, our approach is 4.5 times faster than prior tracking algorithms on the MOT benchmark and we are state-of-the-art in dense crowd videos by over 2.6% on the absolute scale on average.

==> table2.tex <==
\begin{table}[!htb]
  \centering
  \resizebox{\columnwidth}{!}{%
%   \scalebox{0.9}{
  \begin{tabular}{|c|c|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1.5cm}|p{1.5cm}|p{1cm}|}
  \hline
  Dataset & Tracker  ? & FPS$\uparrow$ & FN$\downarrow$ & MT(\%)$\uparrow$ & ML(\%)$\downarrow$ & MOTA(\%)$\uparrow$ & MOTP(\%)$\uparrow$  & IDSW$\downarrow$\\    \hline
     & SMOT \cite{smot}  & 2.7 & 5,172 & 6.3 & 25.0 & 6.7 & 71.4 & 221  \\
    % \cline{2-11}
%   \multirow{2}{*}{Adl-Rundle-1} & CEM \cite{cem-lin2} & No  & 1.1 & 4,465 & 21.9 & 12.5 & 9.2 & 71.4 & 82  \\
  \multirow{2}{*}{Adl-Rundle-1} & MotiCon \cite{moticon}    & 1.4 & 4,628 & 18.8 & 12.5 & 1.0 & 70.3 & 136  \\
  & ALExTRAC \cite{alex}   & 3.7 & 5,010 & 15.6 & 21.9 & 5.1 & 71.3 & 321  \\
   & DCO\_X \cite{discrete}   & 0.3 & 4,920 & 15.6 & 28.1 & 10.0 & 72.0 & 68  \\
    \cline{2-9}
    & \textbf{DensePeds}  & \textbf{28.9} & \textbf{4,302} & \textbf{21.8} & \textbf{9.0} & \textbf{31.4} & \textbf{74.0} & \textbf{44}  \\
   \hline
    %  & EDMT & No & Yes & 1.8 & 87,890 & 17 & 39.9 & 45.3 & 75.9 & 639  \\
    % & INTERA\_MOT & No & No & 4.3 & 85,547 & 18.1 & 38.7 & 45.4 & 74.4 & 600  \\
    % & MHT\_DAM & No & Yes & 0.8 & 91,758 & 16.2 & 43.2 & 45.8 & 76.3 & 590  \\
    % \cline{2-11} 
    % & JMC & No & No & 0.8 & 90,914 & 15.5 & 39.7 & 46.3 & 75.7 & 657  \\
    % \cline{2-11} 
    & CEM\_16 \cite{cem-lin2}   & 0.3 & 11,553 & 9.5 & 47.6 & 26.7 & 80.0 & 77  \\
    % \cline{2-11} 
    \multirow{2}{*}{MOT16-08} & SMOT\_16 \cite{smot}  & 0.2 & 11,572 & 1.6 & 44.4 & 20.8 & 78.8 & 315 \\
    & QuadMOT16 \cite{quad}   & 1.8 & 11,072 & 11.1 & 41.3 & 29.9 & 79.4 & 74 \\
    % & GCRA & No & No & 2.8 & 88,586 & 12.9 & 41.1 & 48.2 & 77.5 & 821 \\
    % & LMP & No & No & 0.5 & 86,245 & 18.2 & 40.1 & 48.8 & 79 & 595 \\
    % & TPM & No & No & 0.8 & 83,031 & 20.0 & 38.9 & 49.1 & 74.8 & 679 \\
    \cline{2-9} 
    & \textbf{DensePeds}   & \textbf{18.8} & \textbf{9,898} & \textbf{20.6} & \textbf{36.5} & \textbf{32.7} & \textbf{80.0} & \textbf{63}  \\
  \hline
  \end{tabular}
  }
%   }
  \caption{Evaluation on the MOT benchmark with \textit{offline methods}. Bold is best. Arrows ($\uparrow, \downarrow$) indicate the direction of better performance. Summary: DensePeds is 18X faster than previous methods and improves accuracy by upto 30\%}
  \label{table2}
\end{table}
% \vspace{-10pt}



==> table3.tex <==
\begin{table}[!htb]
  \centering
    \resizebox{\columnwidth}{!}{%
%   \scalebox{0.9}{
  \begin{tabular}{|c|c|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1.5cm}|p{1.5cm}|p{1cm}|}
  \hline
  Dataset & Tracker  & FPS$\uparrow$ & FN$\downarrow$ & MT(\%)$\uparrow$ & ML(\%)$\downarrow$ & MOTA(\%)$\uparrow$ & MOTP(\%)$\uparrow$  & IDSW$\downarrow$\\    \hline
    
    
    \multirow{2}{*}{Adl-Rundle-1} & LFNF \cite{lfnf-lin4} & 4.0 & 5,827 & 9.4 & 25.0 & 17.6 & 73.3 & 94  \\
%   \multirow{2}{*}{Adl-Rundle-1} & MHT\_DAM &  No & Yes & 0.7 & 32,060 & 16.0 & 43.8 & 32.4 & 71.8 & 435  \\
    %  & LFNF &  No & Yes & 4.0 & 35,095 & 9.6 & 41.7 & 31.6 & 72.0 & 961  \\
    %  \cline{2-11}
    %  \multirow{2}{*}{Adl-Rundle-1}  &\textbf{DensePeds-withoutFRVO} & Yes & Yes & \textbf{18.8} & \textbf{78,413} & \textbf{20.3} & \textbf{36.1} & 40.9 & 75.5 & 722  \\
      \cline{2-9}
   & \textbf{DensePeds}  & \textbf{28.9} & \textbf{4,302} & \textbf{21.8} & \textbf{9.0} & \textbf{31.4} & \textbf{74.0} & \textbf{44}  \\
    
    
    
     \hline
    
    
    
    %  & EDMT & No & Yes & 1.8 & 87,890 & 17 & 39.9 & 45.3 & 75.9 & 639  \\
    \multirow{2}{*}{MOT16-08} & CEM\_16 \cite{cem-lin2}  & 0.3 & 11,553 & 9.5 & 47.6 & 26.7 & 80.0 & 77  \\
    %  \multirow{2}{*}{MOT16-08} & MHT\_DAM & No & Yes & 0.8 & 91,758 & 16.2 & 43.2 & 45.8 & 76.3 & 590  \\
    %  & LFNF16 & No & Yes & 0.6 & 95,363 & 13.3 & 45.7 & 43.6 & 76.6 & 836  \\
     \cline{2-9} 
    %   \multirow{2}{*}{MOT16-08} &\textbf{DensePeds-Lin} & Yes & Yes & \textbf{18.8} & \textbf{78,413} & \textbf{20.3} & \textbf{36.1} & 40.9 & 75.5 & 722  \\
    %   \cline{2-11}
    & \textbf{DensePeds} & \textbf{18.8} & \textbf{9,898} & \textbf{20.6} & \textbf{36.5} & \textbf{32.7} & \textbf{80.0} & \textbf{63}  \\
     \hline
  \end{tabular}
  }
  \caption{Evaluation on the MOT benchmark with \textit{linear motion-model based tracking methods, LFNF and CEM\_16}. This highlights the benefits of our DensePeds algorithm, which is based on FRVO and sparse feature vector computation. Bold is best. Arrows ($\uparrow, \downarrow$) indicate the direction of better performance. Summary: DensePeds is 18X faster than previous methods and improves accuracy by upto 13\%}
  \label{table3}
\end{table}

% \input{AuthorKit19/LaTeX/dense.tex}

